Expert-aware uncertainty estimation for quality control of neural-based blood typing

In medical diagnostics, accurate uncertainty estimation for neural-based models is essential for complementing second-opinion systems. Despite neural network ensembles' proficiency in this problem, a gap persists between actual uncertainties and predicted estimates. A major difficulty here is the lack of labels on the hardness of examples: a typical dataset includes only ground truth target labels, making the uncertainty estimation problem almost unsupervised. Our novel approach narrows this gap by integrating expert assessments of case complexity into the neural network's learning process, utilizing both definitive target labels and supplementary complexity ratings. We validate our methodology for blood typing, leveraging a new dataset "BloodyWell" unique in augmenting labeled reaction images with complexity scores from six medical specialists. Experiments demonstrate enhancement of our approach in uncertainty prediction, achieving a 2.5-fold improvement with expert labels and a 35% increase in performance with estimates of neural-based expert consensus.

==> chapters/experts.tex <==
\section{Experts' assessment of uncertainty}
\label{sec:experts}

Medical experts' extensive problem-solving experience enhances their ability to evaluate the complexity of various cases accurately. 
Assuming that experts have encountered diverse data variations, their assessments primarily reflect aleatoric uncertainty inherent in the data rather than uncertainties associated with a classifier itself. 
This implies that expert evaluations could reliably indicate uncertainty levels applicable to both human and algorithmic classifiers. 
Moreover, experts' answers are calibrated, as they aim at estimating the probability of an error.

Total uncertainty consists of the sum of aleatoric and epistemic uncertainty~\cite{gawlikowski2023survey}.
Thus, when the classifier is a neural network, the epistemic component of uncertainty must also be evaluated.
An outsider is bad at estimating a neural network's uncertainty, while it is possible for a neural network per se. 
Therefore, our idea is to combine an estimate of the neural network's epistemic uncertainty with an estimate of the experts' aleatoric uncertainty, covering all possible uncertainty sources.

We adopted a straightforward way for expert evaluation.
For binary classification assessment, $k$-th expert selected reaction probabilities $e_k$ from $0.00$ (definitely negative reaction), $0.25$ (most likely negative), $0.50$ (difficult to answer), $0.75$ (most likely positive), and $1.00$ (definitely positive).
In our work, the aleatoric uncertainty as the distance of the average experts' probability $\overline{e} = \frac1n\sum_{k=1}^{n} e_k$ to the nearest integer:
\begin{equation}
    UQ_{\mathrm{aleatoric}} = \bigg{|}[\overline{e}] - \overline{e} \bigg{|},
\end{equation}
extending the notion of the maximum probability confidence estimate.
Such a metric conserves the same order of uncertainties as entropy, which is commonly used for aleatoric uncertainty estimation~\cite{mukhoti2023deep}.
To evaluate epistemic uncertainty, we adopted approaches discussed in subsequent sections.

\begin{figure}  
    \centering
    \includegraphics[width=0.7\textwidth]{images/mistakes_highlight.eps}
        \caption{
        } \label{fig:mistakes}
\end{figure}
